Asymptotic Freeness of Layerwise Jacobians Caused by Invariance of Multilayer Perceptron: The Haar Orthogonal Case

Free Probability Theory (FPT) provides rich knowledge for handling mathematical difficulties caused by random matrices that appear in research related to deep neural networks (DNNs), such as the dynamical isometry, Fisher information matrix, and training dynamics. FPT suits these researches because the DNN's parameter-Jacobian and input-Jacobian are polynomials of layerwise Jacobians. However, the critical assumption of asymptotic freenss of the layerwise Jacobian has not been proven completely so far. The asymptotic freeness assumption plays a fundamental role when propagating spectral distributions through the layers. Haar distributed orthogonal matrices are essential for achieving dynamical isometry. In this work, we prove asymptotic freeness of layerwise Jacobians of multilayer perceptron (MLP) in this case. A key of the proof is an invariance of the MLP. Considering the orthogonal matrices that fix the hidden units in each layer, we replace each layer's parameter matrix with itself multiplied by the orthogonal matrix, and then the MLP does not change. Furthermore, if the original weights are Haar orthogonal, the Jacobian is also unchanged by this replacement. Lastly, we can replace each weight with a Haar orthogonal random matrix independent of the Jacobian of the activation function using this key fact.

==> mycommand.tex <==
%%% common
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\Q}{\mathbb Q}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\F}{\mathbb F}
\newcommand{\K}{\mathbb K}

\newcommand{\E}{\mathbb E}  % Expectation
\renewcommand{\O}[1]{\mathbf O_{#1}} %% Orthogonal Group


\newcommand{\ms}[1]{\mathscr{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\eu}[1]{\EuScript{#1}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}

\newcommand{\bs}[1]{\boldsymbol{#1}}

\newcommand{\eps}{\varepsilon}


\DeclareMathOperator{\tr}{\mathrm{tr}}
\DeclareMathOperator{\Tr}{\mathrm{Tr}}
\DeclareMathOperator{\supp}{\sigma}
\DeclareMathOperator{\rank}{\mathrm{rank}}
\DeclareMathOperator{\diag}{\mathrm{diag}}

\DeclareMathOperator{\Normal}{\mathcal{N}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\ESD}{ESD}

\newcommand{\freeas}[1]{\coprod^{\text{F~a.s.}}_{#1\to \infty}}

%%% operatinos
\newcommand{\To}{\Rightarrow}
\newcommand{\pp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\abs}[1]{|#1|}
%%% MLP
\newcommand{\pre}{h}
\newcommand{\post}{x}
\newcommand{\act}{\varphi}


%%% free version of NTK
\newcommand{\FNTK}{\Xi^\Box}
\newcommand{\fdelta}{\delta^\Box}
\newcommand{\fda}{d}  %%% infinite-dimensional limit of D.

\newcommand{\Hmltn}{H}

\newcommand{\affine}[2]{ ( #2 +  #1 \,\boldsymbol{\cdot}\, )_*}




\newcommand{\embedding}[1]{ \begin{pmatrix} #1 & 0 \\ 0 & 0 \end{pmatrix}}
\newcommand{\entries}{\sim^\mathrm{entries}}




==> mytikz.tex <==
\usepackage{tikz}
%\usepackage{amsfonts}
%\usepackage{amsmath,amssymb}
\usepackage{systeme,mathtools}
\usetikzlibrary{positioning,arrows.meta,quotes,automata}
\usetikzlibrary{shapes,snakes}
\usetikzlibrary{bayesnet}

\tikzset{>=latex}
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south]


\tikzset{circ/.style={
    circle,
    draw=black,
    fill=white,
    inner sep=0pt,
    minimum size=1cm,
    }
}



\tikzset{box/.style={
    rectangle,
    draw=black,
    fill=white,
    inner sep=0pt,
    minimum size=1cm,
    }
}


\tikzset{empty style/.style={
    circle,
    draw=white,
    fill=white,
    inner sep=0pt,
    minimum size=0.6cm
    }
}



\tikzset{mark style/.style={
    mark size=1pt,
    color=black
    }
}    
\tikzset{text style/.style={
    text width=0.5cm
    }
}



